Reanalysis of the X-ray burst associated FRB 200428 with Insight-HXMT observations

A double-peak X-ray burst from the Galactic magnetar SGR J1935+2154 was discovered as associated with the two radio pulses of FRB 200428 separated by 28.97+-0.02 ms. Precise measurements of the timing and spectral properties of the X-ray bursts are helpful for understanding the physical origin of fast radio bursts (FRBs). In this paper, we have reconstructed some information about the hard X-ray events, which were lost because the High Energy X-ray Telescope (HE) onboard the Insight-HXMT mission was saturated by this extremely bright burst, and used the information to improve the temporal and spectral analyses of the X-ray burst. The arrival times of the two X-ray peaks by fitting the new Insight-HXMT/HE lightcurve with multi-Gaussian profiles are 2.77+-0.45 ms and 34.30+-0.56 ms after the first peak of FRB 200428, respectively, while these two parameters are 2.57+-0.52 ms and 32.5+-1.4 ms if the fitting profile is a fast rise and exponential decay function. The spectrum of the two X-ray peaks could be described by a cutoff power-law with cutoff energy ~60 keV and photon index ~1.4, the latter is softer than that of the underlying bright and broader X-ray burst when the two X-ray peaks appeared.

==> ref1.tex <==
\begin{thebibliography}{10}

%\setcounter{enumiv}{30}



\bibitem{Petroff2019}
E.~{Petroff}, J.~W.~T.~{Hessels}, D.~R.~{Lorimer}, Fast radio bursts. 
{\it Astronomy and Astrophysics Review\/}. {\bf 27}, 4 (2019).
%Fast radio bursts

\bibitem{Cordes2019}
J.~M.~{Cordes}, S.~{Chatterjee}, Fast radio bursts: an extragalactic enigma. 
{\it Annual Review of Astronomy and Astrophysics\/}. {\bf 57}, 417 (2019).
%Fast Radio Bursts: An Extragalactic Enigma




\bibitem{Xiao21}
D.~{Xiao}, F. Y.~{Wang}, Z. G.~{Dai}, The physics of fast radio bursts. 
{\it Science China Physics, Mechanics, and Astronomy\/} {\bf 64}, 249501 (2021).
%The physics of fast radio bursts

\bibitem{Zhang20}
B.~{Zhang}, The physical mechanisms of fast radio bursts.
{\it Nature\/} {\bf 587}, 45 (2020).
%The physical mechanisms of fast radio bursts



\bibitem{chime2020a}
The CHIME/FRB Collaboration: B.~C.~{Anderson}, K.~M.~{Bhardwaj}, A.~{Bij}, {\it et~al.\/}, A bright millisecond-duration radio burst from a Galactic magnetar. 
{\it Nature\/} {\bf 587}, 54 (2020).
%A bright millisecond-duration radio burst from a Galactic magnetar

\bibitem{Bochenek20}
C.~D.~{Bochenek}, V.~{Ravi}, K.~V.~{Belov}, {\it et~al.\/}, A fast radio burst associated with a Galactic magnetar. 
{\it Nature\/} {\bf 587}, 59 (2020).
%A fast radio burst associated with a Galactic magnetar


%---------------------------------------------------------%


\bibitem{zhangsn2020}
S.-N.~{Zhang}, T.~P.~{Li}, F. J.~{Lu}, {\it et~al.\/}, Overview to the Hard X-ray Modulation Telescope (\textit{Insight}-HXMT) Satellite. 
{\it Science China Physics, Mechanics, and Astronomy\/} {\bf 63}, 249502 (2020).
%{Overview to the Hard X-ray Modulation Telescope (\textit{Insight}-HXMT) Satellite}


\bibitem{S.Zhang..2018}
S.~{Zhang}, N. S.~{Zhang}, F. J.~{Lu}, {\it et~al.\/}, The \textit{Insight}-HXMT mission and its recent progresses. 
In {\it Proc. SPIE\/}, vol.~{\bf 10699} of {\it Society of Photo-Optical Instrumentation Engineers (SPIE) Conference Series}, 106991U (2018).
%{The \textit{Insight}-HXMT mission and its recent progresses}


\bibitem{li2020flight}
X.-B.~{Li}, X.-F.~{Li}, Y.~{Tan}, {\it et~al.\/}, In-flight calibration of the \textit{Insight}-Hard X-ray Modulation Telescope. 
{\it Journal of High Energy Astrophysics\/} {\bf 27}, 64 (2020).
%{In-flight calibration of the \textit{Insight}-Hard X-ray Modulation Telescope}


%-----------------------------------------------

%------------------------------------------------%

\bibitem{hxmt2020}
S.~N.~{Zhang}, S.~L.~{Xiong}, C.~K.~{Li}, {\it et~al.\/}, \textit{Insight}-HXMT X-ray and hard X-ray detection of the double peaks of the fast radio burst from SGR 1935+2154. 
{\it The Astronomer's Telegram\/} {\bf 13696}, 1 (2020).
%\textit{Insight}-HXMT X-ray and hard X-ray detection of the double peaks of the Fast Radio Burst from SGR 1935+2154

\bibitem{hxmt2020a}
C.~K.~{Li}, L.~{Lin}, S.~L.~{Xiong}, {\it et~al.\/}, HXMT identification of a non-thermal X-ray burst from SGR J1935+2154 and with FRB 200428. 
{\it Nat. Astron.\/} {\bf 5}, 378 (2021).
%HXMT identification of a non-thermal X-ray burst from SGR J1935+2154 and with FRB 200428

\bibitem{kw2020a}
A.~{Ridnaia}, D.~{Svinkin}, D.~{Frederiks}, {\it et~al.\/}, A peculiar hard X-ray counterpart of a Galactic fast radio burst. 
{\it Nat. Astron.\/} {\bf 5}, 372 (2021).
%A peculiar hard X-ray counterpart of a Galactic fast radio burst

\bibitem{in2020a}
S.~{Mereghetti}, V.~{Savchenko}, C.~{Ferrigno}, {\it et~al.\/}, INTEGRAL discovery of a burst with associated radio emission from the magnetar SGR 1935+2154. 
{\it \apjl\/} {\bf 898}, L29 (2020).
%INTEGRAL discovery of a burst with associated radio emission from the magnetar SGR 1935+2154

%------------------------------------------------%


\bibitem{Wu2020}
Q.~{Wu}, G.~Q.~{Zhang}, F.~Y.~{Wang},  Z. G.~{Dai}, Understanding FRB 200428 in the synchrotron maser shock model: consistency and possible challenge.
{\it \apjl\/} {\bf 900}, L26 (2020).
%Understanding FRB 200428 in the synchrotron maser shock model: consistency and possible challenge

\bibitem{Margalit2019}
B.~{Margalit}, E.~{Berger}, B.~D.~{Metzger}, Fast radio bursts from magnetars born in binary neutron star mergers and accretion induced collapse.
{\it \apj\/} {\bf 886}, 110 (2019).
%Fast Radio Bursts from Magnetars Born in Binary Neutron Star Mergers and Accretion Induced Collapse

\bibitem{Xiao21b}
D.~{Xiao}, Z.-G.~{Dai}, Double-peaked pulse profile of FRB 200428: synchrotron maser emission from magnetized shocks encountering a density jump. 
{\it \apjl.\/} {\bf 904}, L5 (2020).
%Double-peaked Pulse Profile of FRB 200428: Synchrotron Maser Emission from Magnetized Shocks Encountering a Density Jump

\bibitem{Margalit2020}
B.~{Margalit}, P.~{Beniamini}, N.~{Sridhar}, B.~D.~{Metzger}, {\it et~al.\/}, Implications of a ``fast radio burst" from a galactic magnetar. 
{\it \apjl\/} {\bf 899}, L27 (2020).
%Implications of a ``Fast Radio Burst" from a Galactic Magnetar

\bibitem{Yu2020}
Y.-W.~{Yu}, Y.-C.~{Zhou}, Z.-G.~{Dai}, W.-F.~{Yu}, The confrontation of the shock-powered synchrotron maser model with the Galactic FRB 200428. 
{\it \mnras\/} {\bf 500}, 2704 (2021).
%The confrontation of the shock-powered synchrotron maser model with the Galactic FRB 200428

\bibitem{Yuan2020}
Yajie.~{Yuan}, Andrei~M.~{Beloborodov}, Alexander~Y.~{Chen}, Yuri.~{Levin}, Plasmoid ejection by Alfvén waves and the fast radio bursts from SGR 1935+2154.
{\it \apjl\/} {\bf 900}, L21 (2020).
%Plasmoid ejection by Alfvén waves and the fast radio bursts from SGR 1935+2154

\bibitem{Wadiasingh2019}
Z.~{Wadiasingh}, A.~{Timokhin}, Repeating fast radio bursts from magnetars with low magnetospheric twist. 
{\it \apj\/} {\bf 879}, 4 (2019).
%Repeating Fast Radio Bursts from Magnetars with Low Magnetospheric Twist

\bibitem{Kumar2020}
P.~{Kumar}, Z.~{Bosnjak}, FRB coherent emission from decay of Alfv$\acute{\rm{e}}$n waves. 
{\it \mnras\/} {\bf 494}, 2385 (2020).
%FRB coherent emission from decay of Alfv$\acute{\rm{e}}$n waves

\bibitem{Yang2020}
Y.-P.~{Yang}, J.-P.~{Zhu}, B.~{Zhang}, X.-F.~{Wu}, Pair separation in parallel electric field in magnetar magnetosphere and narrow spectra of fast radio bursts. 
{\it \apjl\/} {\bf 901}, L13 (2020).
%{Pair Separation in Parallel Electric Field in Magnetar Magnetosphere and Narrow Spectra of Fast Radio Bursts}

\bibitem{Lu2020}
W.~B.~{Lu}, P.~{Kumar}, B.~{Zhang}, A unified picture of galactic and cosmological fast radio bursts. 
{\it \mnras\/} {\bf 498}, 1397 (2020).
%A unified picture of Galactic and cosmological fast radio bursts

\bibitem{Yang21}
Y.-P.~{Yang}, B.~{Zhang}, Fast radio bursts and their high-energy counterpart from magnetar magnetospheres. 
{\it arXiv:\/} 2104.01925%{\bf 498}, 1397 (2020).
%Fast radio bursts and their high-energy counterpart from magnetar magnetospheres

\bibitem{Dai2020}
Z.~G.~{Dai}, A magnetar-asteroid impact model for FRB 200428 associated with an X-ray burst from SGR 1935+2154. 
{\it \apjl\/} {\bf 897}, L40 (2020).
%A Magnetar-asteroid Impact Model for FRB 200428 Associated with an X-Ray Burst from SGR 1935+2154


\bibitem{Ceng2020}
J.~J.~{Geng}, B.~{Li}, L.-B.~{Li}, {\it et~al.\/}, FRB 200428: an impact between an asteroid and a magnetar. 
{\it \apjl\/} {\bf 898}, L55 (2020).
%FRB 200428: an impact between an asteroid and a magnetar


\bibitem{Wang2020}
W.-Y.~{Wang}, R.~{Xu}, and X.~{Chen}, On the Magnetospheric Origin of Repeating Fast Radio Bursts. 
{\it \apj\/} {\bf 899}, 109 (2020).
%FRB 200428: an impact between an asteroid and a magnetar



\bibitem{Weinberg72}
S.~Weinberg, 
{\it ``Gravitation and cosmology: principles and application of the general theory of relativity"}, (John Wiley \& Sons, New York U.S.A., 1972).


\bibitem{Gabler2018}
M.~{Gabler}, P.~{Cerd$\acute{\textit{a}}$-Dur$\acute{\textit{a}}$n}, N.~{Stergioulas}, {\it et~al.\/}, Constraining properties of high-density matter in neutron stars with magneto-elastic oscillations. 
{\it \mnras\/} {\bf 476}, 4199 (2018).
%Constraining properties of high-density matter in neutron stars with magneto-elastic oscillations





\bibitem{Israel16}
G.~L.~{Israel}, P.~{Esposito}, N.~{Rea}, The discovery, monitoring and environment of SGR J1935+2154. 
{\it \mnras\/} {\bf 457}, 3448 (2016).
%The discovery, monitoring and environment of SGR J1935+2154



\bibitem{Zhang13}
S.~N.~{Zhang}, Black hole binaries and microquasars. 
{\it Frontiers of Physics\/} {\bf 8}, 630 (2013).
%The discovery, monitoring and environment of SGR J1935+2154





\bibitem{Ruderman75}
M.~A.~{Ruderman}, P.~G.~{Sutherland}, Theory of pulsars: polar gaps, sparks, and coherent microwave radiation. 
{\it \apj\/} {\bf 196}, 51 (1975).
%Theory of pulsars: polar gaps, sparks, and coherent microwave radiation


\bibitem{WJS2020}
J.~S.~{Wang}, The radio/X-ray burst from SGR 1935+2154: radiation mechanisms and the possible QPOs. 
{\it \apj\/} {\bf 900}, 172 (2020). 
%The radio/X-ray burst from SGR 1935+2154: radiation mechanisms and the possible QPOs


\bibitem{Dai2016}
Z.~G.~{Dai}, J.~S.~{Wang}, X.~F.~{Wu}, Y.~F.~{Huang}, Repeating fast radio bursts from highly magnetized pulsars traveling through asteroid belts. 
{\it \apj\/} {\bf 829}, 27 (2016).
%Repeating Fast Radio Bursts from Highly Magnetized Pulsars Travelling through Asteroid Belts



%-----------------------------------------------

\bibitem{Thompson1996}
C.~{Thompson}, R.~C.~{Duncan}, The soft gamma repeaters as very strongly magnetized neutron stars. II. Quiescent neutrino, X-ray, and Alfv$\acute{\rm{e}}$n wave emission. 
{\it \apj\/} {\bf 473}, 322 (1996).
%{The Soft Gamma Repeaters as Very Strongly Magnetized Neutron Stars. II. Quiescent Neutrino, X-Ray, and Alfv$\acute{\rm{e}}$n Wave Emission}




\bibitem{Geng2015}
J.-J.~{Geng}, Y.-F.~{Huang}, Fast radio bursts: collisions between neutron stars and asteroids/comets. 
{\it \apj\/} {\bf 809}, 24 (2015).
%{{Fast Radio Bursts: Collisions between Neutron Stars and Asteroids/Comets}



\bibitem{Link16}
B.~{Link}, C.~A.~{van Eysden}, Torsional oscillations of a magnetar with a tangled magnetic field. 
{\it \apjl\/} {\bf 823}, L1 (2016).
%{Torsional oscillations of a magnetar with a tangled magnetic field}


\bibitem{Braithwaite09}
J.~{Braithwaite}, Axisymmetric magnetic fields in stars: relative strengths of poloidal and toroidal components. 
{\it \mnras\/} {\bf 397}, 763 (2009).
%{Axisymmetric magnetic fields in stars: relative strengths of poloidal and toroidal components}


\bibitem{Zhou20}
P.~{Zhou}, X.~{Zhou}, Y.~{Chen}, {\it et~al.\/}, Revisiting the distance, environment, and supernova properties of SNR G57.2+0.8 that hosts SGR 1935+2154. 
{\it \apj\/} {\bf 905}, 99 (2020).
%{Revisiting the Distance, Environment, and Supernova Properties of SNR G57.2+0.8 that Hosts SGR 1935+2154}


\bibitem{Zhong20}
S.-Q.~{Zhong}, Z.-G.~{Dai}, H.-M.~{Zhang}, C.-M.~{Deng}, On the distance of SGR 1935+2154 associated with FRB 200428 and hosted in SNR G57.2+0.8. 
{\it \apjl\/} {\bf 898}, L5 (2020).
%{On the Distance of SGR 1935+2154 Associated with FRB 200428 and Hosted in SNR G57.2+0.8}


\bibitem{Kothes18}
R.~{Kothes}, X.~{Sun}, B.~{Gaensler}, W. {Reich}, A radio continuum and polarization study of SNR G57.2+0.8 associated with magnetar SGR 1935+2154.
{\it \apj\/} {\bf 852}, 54 (2018).
%{A Radio Continuum and Polarization Study of SNR G57.2+0.8 Associated with Magnetar SGR 1935+2154}

\bibitem{Lin20a}
L.~{Lin}, E.~{Gogus}, O.~J. {Roberts}, {\it et~al.\/}, Burst properties of the most recurring transient magnetar SGR J1935+2154. 
{\it \apj\/} {\bf 893}, 156 (2020).
%{Burst Properties of the Most Recurring Transient Magnetar SGR J1935+2154}





\bibitem{Lin20b}
L.~{Lin}, E.~{Gogus}, O.~J. {Roberts}, {\it et~al.\/}, Fermi/GBM view of the 2019 and 2020 burst active episodes of SGR J1935+2154. 
{\it \apjl\/} {\bf 902}, L43 (2020).
%{Fermi/GBM View of the 2019 and 2020 Burst Active Episodes of SGR J1935+2154}


\bibitem{Gold69}
P.~{Goldreich}, W.~H.~{Julian},  Pulsar electrodynamics.
{\it \apj\/} {\bf 157}, 869 (1969).
%{Pulsar Electrodynamics}



\bibitem{Yue07}
Y.~L.~{Yue}, R.~X.~{Xu}, What can the braking indices tell us about the nature of pulsars ?
{\it Advances in Space Research\/} {\bf 40}, Issue 10, 1491 (2007).
%{What can the braking indices tell us about the nature of pulsars ?}

\bibitem{Tong15}
F.~F.~{Kou}, H.~{Tong}, Rotational evolution of the Crab pulsar in the wind braking model. 
{\it \mnras\/} {\bf 450}, 1990 (2015).
%{Rotational evolution of the Crab pulsar in the wind braking model}




\bibitem{Zhang19}
B.~{Zhang}, 
{\it ``The Physics of Gamma-Ray Bursts"} (Cambridge University Press, United Kingdom, 2019).
%{The Physics of Gamma-Ray Bursts}


\bibitem{Vink20}
J.~{Vink}, 
{\it``Physics and Evolution of Supernova Remnants"},  (Springer Nature Switzerland AG, Cham, Switzerland, 2020).
%{Physics and Evolution of Supernova Remnants


\bibitem{Younes21}
G.~{Younes}, T.~{Guver}, C.~{Kouveliotou}, {\it et~al.\/}, NICER View of the 2020 burst storm and persistent emission of SGR 1935+2154. 
{\it \apjl\/} {\bf 904}, L21 (2020).
%{NICER View of the 2020 Burst Storm and Persistent Emission of SGR 1935+2154}



\bibitem{Beniamini20}
P.~{Beniamini}, P.~{Kumar}, What does FRB light-curve variability tell us about the emission mechanism? 
{\it \mnras\/} {\bf 498}, 651 (2020).
%What does FRB light-curve variability tell us about the emission mechanism


\bibitem{Schwartz14}
M.~{Schwartz}, 
{\it ``Quantum Field Theory and the Standard Model"}, (Cambridge University Press, United Kingdom, 2014).
%Quantum Field Theory and the Standard Model




\end{thebibliography}

